Deformable Graph Convolutional Networks

Graph neural networks (GNNs) have significantly improved the representation power for graph-structured data. Despite of the recent success of GNNs, the graph convolution in most GNNs have two limitations. Since the graph convolution is performed in a small local neighborhood on the input graph, it is inherently incapable to capture long-range dependencies between distance nodes. In addition, when a node has neighbors that belong to different classes, i.e., heterophily, the aggregated messages from them often negatively affect representation learning. To address the two common problems of graph convolution, in this paper, we propose Deformable Graph Convolutional Networks (Deformable GCNs) that adaptively perform convolution in multiple latent spaces and capture short/long-range dependencies between nodes. Separated from node representations (features), our framework simultaneously learns the node positional embeddings (coordinates) to determine the relations between nodes in an end-to-end fashion. Depending on node position, the convolution kernels are deformed by deformation vectors and apply different transformations to its neighbor nodes. Our extensive experiments demonstrate that Deformable GCNs flexibly handles the heterophily and achieve the best performance in node classification tasks on six heterophilic graph datasets.

==> Algorithms/pseudocode.tex <==
\begin{algorithm}[t]
  \caption{Our network (Temp)}
  \label{alg:pseudocode}
\begin{algorithmic}[1]
%   \REQUIRE $G$, $\mathbf{X} \in \mathbf{R}^{n \times d}$\\
%   \textbf{Network Parameters:} $\mathbf{W}_e \in \mathbf{R}^{d \times d_e}, \mathbf{W}_o \in \mathbf{R}^{d_e \times C}, \alpha^{(k)}, \text{weight of MLP layers}$
%   \ENSURE $\mathbf{h}_i^{(\text{output})} (i=1, \dots, n)$
%   \FOR{$v_u \in V$}
    \STATE $\eb_{i,0} \leftarrow \xb_i \quad \forall i \in V$
    \STATE $\Gc_0 \leftarrow \text{KNN}\left(\left\{\eb_{i,0},\forall i \in V \right\}, k \right)$
    \FOR{$c=1$ {\bfseries to} $c=C$}
        \STATE $\eb_{i,c} \leftarrow \frac{1}{\text{deg}\left(i \right)}\sum_{j \in \Nc\left(i\right)}\eb_{j,c-1}$
        \STATE $\Gc_c \leftarrow \text{KNN}\left(\left\{\eb_{i,c}, \forall i \in V  \right\}, k\right)$
    \ENDFOR
    \STATE $\Gc_{C+1} \leftarrow \mathcal{G}$
    
    \STATE $\hb_i \leftarrow \sigma \left(\Wb \xb_i + \bb \right), \forall i \in V$
    \FOR{$c=0$ {\bfseries to} $c=C+1$}
        \FOR{$i \in \left\{u\right\} \cup \left\{v : \left(u,v\right) \in \Gc_c\right\}$}
            \STATE $\mathbf{q}_{i,c} \leftarrow \mathbf{Q}_{c}\mathbf{e}_{i,c}/ \lVert \mathbf{Q}_{c}\mathbf{e}_{i,c}\rVert_2$
            \STATE $\mathbf{k}_{i,c} \leftarrow \mathbf{K}_c \mathbf{e}_{i,c} / \lVert \mathbf{K}_c \mathbf{e}_{i,c}\rVert_2$
        \ENDFOR
        \FOR{$j \in \Nc_c\left(i \right)$}
            \STATE $a_{j,c} \leftarrow \qb_{i,c}^\top \kb_{j,c}$
            \STATE $p_{j,c} \leftarrow \frac{\exp \left(a_{j,c} \right)}{\sum_{j^\prime \in \Nc_c\left(i \right)} \exp\left(a_{j^\prime,c} \right)}$
            \STATE $\hb_{i,c} \leftarrow \sum_{j \in \Nc_c\left(i\right)} p_{j,c}\Wb_c\hb_{j}$
        \ENDFOR
    \ENDFOR
    \STATE $\mathbf{\tilde{h}}_{i,c} \leftarrow \mathbf{h}_{i,c} / \lVert \mathbf{h}_{i,c}\rVert_2$
    \STATE $s_{i,c} \leftarrow \frac{\exp \left(\mathbf{z}_s^\top \mathbf{\tilde{h}}_{i,c} \right)}{\sum_{c^\prime=0}^{C+1} \exp \left(\mathbf{z}_s^\top \mathbf{\tilde{h}}_{i,c^\prime}\right)}$
    \STATE $\mathbf{\hat{h}}_i \leftarrow \sum_{c=0}^{C+1} s_{i,c}\mathbf{\tilde{h}}_{i,c}$
\end{algorithmic}
\end{algorithm}




% \begin{algorithm}[t]
%   \caption{Our network (Temp)}
%   \label{alg:pseudocode}
% \begin{algorithmic}[1]
% %   \REQUIRE $G$, $\mathbf{X} \in \mathbf{R}^{n \times d}$\\
% %   \textbf{Network Parameters:} $\mathbf{W}_e \in \mathbf{R}^{d \times d_e}, \mathbf{W}_o \in \mathbf{R}^{d_e \times C}, \alpha^{(k)}, \text{weight of MLP layers}$
% %   \ENSURE $\mathbf{h}_i^{(\text{output})} (i=1, \dots, n)$
% %   \FOR{$v_u \in V$}
%     \STATE $\mathbf{\tilde{z}}_i \leftarrow f\left(v_i \right) \quad \forall i\in V$
%     \STATE $[p_{i,1}\dots p_{i,K}] \leftarrow \text{softmax}\left(\mathbf{W}^\top\mathbf{\tilde{z}}_{i} \right) \quad \forall i \in V$
%     \STATE $\mathbf{\tilde{a}}_k \leftarrow {\sum_{i}p_{i,k}\mathbf{\tilde{z}}_i}/{\sum_{i}p_{i,k}}$
%     \FOR{$l=0$ {\bfseries to} $l=L-1$}
%         \STATE $\mathbf{a}_k^{(l)} \leftarrow {\sum_{i}p_{i,k}\mathbf{h}^{(l)}_i}/{\sum_{i}p_{i,k}}$
%         \STATE $\mathbf{c}_{i,k}^{(l+1)} \leftarrow \sum_{u \in \mathcal{N}(v)} \frac{\exp  \left(\mathbf{z}_u^\top \mathbf{a}_k \right)}{\sum_{k^\prime}\exp\left(\mathbf{z}_u^\top \mathbf{a}_{k^\prime} \right)} \mathbf{W}_k \mathbf{h}_u^{(l)}$
%         \STATE $\mathbf{n}_i^{(l+1)} \leftarrow \sum_k \mathbf{c}_{i,k}^{(l+1)}$
%         \STATE $\mathbf{e}_i^{(l+1)} \leftarrow \sum_k \frac{\exp  \left(\mathbf{z}_i^\top \mathbf{a}_k \right)}{\sum_{k^\prime}\exp\left(\mathbf{z}_i^\top \mathbf{a}_{k^\prime} \right)}\mathbf{W}^\prime \mathbf{a}_k^{(l)}$
%         \STATE $\mathbf{h_i}^{(l+1)} \leftarrow \mathbf{n}_i^{(l+1)} + \mathbf{e}_i^{(l+1)}$
%   \ENDFOR
% \end{algorithmic}
% \end{algorithm}

==> Algorithms/pseudocode2.tex <==
\begin{algorithm}[t]
  \caption{Our network (Temp2)}
  \label{alg:pseudocode}
\begin{algorithmic}[1]
%   \REQUIRE $G$, $\mathbf{X} \in \mathbf{R}^{n \times d}$\\
%   \textbf{Network Parameters:} $\mathbf{W}_e \in \mathbf{R}^{d \times d_e}, \mathbf{W}_o \in \mathbf{R}^{d_e \times C}, \alpha^{(k)}, \text{weight of MLP layers}$
%   \ENSURE $\mathbf{h}_i^{(\text{output})} (i=1, \dots, n)$
%   \FOR{$v_u \in V$}
    \STATE $\eb_{i,0} \leftarrow \xb_i \quad \forall i \in V$
    \STATE $\Gc_0 \leftarrow \text{KNN}\left(\left\{\eb_{i,0},\forall i \in V \right\}, k \right)$
    \FOR{$c=1$ {\bfseries to} $c=C$}
        \STATE $\eb_{i,c} \leftarrow \frac{1}{\text{deg}\left(i \right)}\sum_{j \in \Nc\left(i\right)}\eb_{j,c-1}$
        \STATE $\Gc_c \leftarrow \text{KNN}\left(\left\{\eb_{i,c} \right\}, k\right)$
    \ENDFOR
    \STATE $\Gc_{C+1} \leftarrow \mathcal{G}$
    
    \STATE $\hb_i \leftarrow \sigma \left(\Wb \xb_i + \bb \right), \forall i \in V$
    \FOR{$c=0$ {\bfseries to} $c=C+1$}
        \FOR{$i \in \left\{u\right\} \cup \left\{v : \left(u,v\right) \in \Gc_c\right\}$}
            \STATE $\phi_{i,c} \leftarrow \mathbf{K}_c \mathbf{e}_{i,c} / \lVert \mathbf{K}_c \mathbf{e}_{i,c}\rVert_2$
            \STATE $\tilde{\phi}_k \leftarrow \tilde{\mathbf{Q}}_{k,c} / \lVert \tilde{\mathbf{Q}}_{k,c} \lVert_2 $
            \FOR{$j \in \Nc_c\left(i \right)$}
            \STATE $ \alpha_{i,j,k,c} \leftarrow \left( \phi_{j,c} - \phi_{i,c}\right)^\top \tilde{\phi}_k$
            \STATE $\alpha_{i,j,k,c} \leftarrow \alpha_{i,j,k,c}/\lVert \alpha_{i,j,k,c}\rVert_2$
            \ENDFOR
            % \STATE $\mathbf{q}_{i,c} \leftarrow \mathbf{Q}_{c}\mathbf{e}_{i,c}/ \lVert \mathbf{Q}_{c}\mathbf{e}_{i,c}\rVert_2$
            % \STATE $\mathbf{k}_{i,c} \leftarrow \mathbf{K}_c \mathbf{e}_{i,c} / \lVert \mathbf{K}_c \mathbf{e}_{i,c}\rVert_2$
            \STATE $\hb_{i,c} \leftarrow \sum_k\sum_{j \in \Nc_{\Gc_{c}{(i)}}} \frac{\exp \left( \alpha_{i,j,k,c} / \tau \right) \Wb_{c,k} \hb_{j}}{\mathbb{Z}}$
            
        \ENDFOR
        % \FOR{$j \in \Nc_c\left(i \right)$}
        %     \STATE $a_{j,c} \leftarrow \qb_{i,c}^\top \kb_{j,c}$
        %     \STATE $p_{j,c} \leftarrow \frac{\exp \left(a_{j,c} \right)}{\sum_{j^\prime \in \Nc_c\left(i \right)} \exp\left(a_{j^\prime,c} \right)}$
        %     \STATE $\hb_{i,c} \leftarrow \sum_{j \in \Nc_c\left(i\right)} p_{j,c}\Wb_c\hb_{j}$
        % \ENDFOR
    \ENDFOR
    \STATE $\mathbf{\tilde{h}}_{i,c} \leftarrow \mathbf{h}_{i,c} / \lVert \mathbf{h}_{i,c}\rVert_2$
    \STATE $s_{i,c} \leftarrow \frac{\exp \left(\mathbf{z}_s^\top \mathbf{\tilde{h}}_{i,c} \right)}{\sum_{c^\prime=0}^{C+1} \exp \left(\mathbf{z}_s^\top \mathbf{\tilde{h}}_{i,c^\prime}\right)}$
    \STATE $\mathbf{\hat{h}}_i \leftarrow \sum_{c=0}^{C+1} s_{i,c}\mathbf{\tilde{h}}_{i,c}$
\end{algorithmic}
\end{algorithm}




% \begin{algorithm}[t]
%   \caption{Our network (Temp)}
%   \label{alg:pseudocode}
% \begin{algorithmic}[1]
% %   \REQUIRE $G$, $\mathbf{X} \in \mathbf{R}^{n \times d}$\\
% %   \textbf{Network Parameters:} $\mathbf{W}_e \in \mathbf{R}^{d \times d_e}, \mathbf{W}_o \in \mathbf{R}^{d_e \times C}, \alpha^{(k)}, \text{weight of MLP layers}$
% %   \ENSURE $\mathbf{h}_i^{(\text{output})} (i=1, \dots, n)$
% %   \FOR{$v_u \in V$}
%     \STATE $\mathbf{\tilde{z}}_i \leftarrow f\left(v_i \right) \quad \forall i\in V$
%     \STATE $[p_{i,1}\dots p_{i,K}] \leftarrow \text{softmax}\left(\mathbf{W}^\top\mathbf{\tilde{z}}_{i} \right) \quad \forall i \in V$
%     \STATE $\mathbf{\tilde{a}}_k \leftarrow {\sum_{i}p_{i,k}\mathbf{\tilde{z}}_i}/{\sum_{i}p_{i,k}}$
%     \FOR{$l=0$ {\bfseries to} $l=L-1$}
%         \STATE $\mathbf{a}_k^{(l)} \leftarrow {\sum_{i}p_{i,k}\mathbf{h}^{(l)}_i}/{\sum_{i}p_{i,k}}$
%         \STATE $\mathbf{c}_{i,k}^{(l+1)} \leftarrow \sum_{u \in \mathcal{N}(v)} \frac{\exp  \left(\mathbf{z}_u^\top \mathbf{a}_k \right)}{\sum_{k^\prime}\exp\left(\mathbf{z}_u^\top \mathbf{a}_{k^\prime} \right)} \mathbf{W}_k \mathbf{h}_u^{(l)}$
%         \STATE $\mathbf{n}_i^{(l+1)} \leftarrow \sum_k \mathbf{c}_{i,k}^{(l+1)}$
%         \STATE $\mathbf{e}_i^{(l+1)} \leftarrow \sum_k \frac{\exp  \left(\mathbf{z}_i^\top \mathbf{a}_k \right)}{\sum_{k^\prime}\exp\left(\mathbf{z}_i^\top \mathbf{a}_{k^\prime} \right)}\mathbf{W}^\prime \mathbf{a}_k^{(l)}$
%         \STATE $\mathbf{h_i}^{(l+1)} \leftarrow \mathbf{n}_i^{(l+1)} + \mathbf{e}_i^{(l+1)}$
%   \ENDFOR
% \end{algorithmic}
% \end{algorithm}

==> Algorithms/pseudocode3.tex <==
\begin{algorithm}[h!]
  \caption{Deformable Graph Convolutional Networks}
  \label{alg:pseudocode}
\begin{algorithmic}[1]
%   \REQUIRE $G$, $\mathbf{X} \in \mathbf{R}^{n \times d}$\\
%   \textbf{Network Parameters:} $\mathbf{W}_e \in \mathbf{R}^{d \times d_e}, \mathbf{W}_o \in \mathbf{R}^{d_e \times C}, \alpha^{(k)}, \text{weight of MLP layers}$
%   \ENSURE $\mathbf{h}_i^{(\text{output})} (i=1, \dots, n)$
%   \FOR{$v_u \in V$}
    \FOR{$l=0$ {\bfseries to} $l=L+1$}
        \STATE $\phib_{v}^{(l)} \leftarrow \Wb_\phi^{(l)} \mathbf{e}_{v}^{(l)} / \lVert \Wb_\phi^{(l)} \mathbf{e}_v^{(l)}\rVert_2$
        \STATE $\widetilde{\phib}_h^{(l)} \leftarrow \widetilde{\phib}_h^{(l)} + \Delta_h^{(l)}\left(\eb_v\right)$
        \FOR{$i \in \left\{v\right\} \cup \left\{u : \left(u,v\right) \in \Ec^{(l)}\right\}$}
            \FOR{$j \in \Nc_c\left(i \right)$}
            \STATE $\rb^{\prime (l)}_{j, i} \leftarrow {\phib_{j}^{(l)} - \phib_{i}^{(l)}}/{\lVert \phib_{j}^{(l)} - \phib_{i}^{(l)} \rVert_2}$
            \STATE $\rb_{j, i}^{(l)} \leftarrow [\rb_{j, i}^{\prime(l)} || 0],\ $ {\bfseries  if} $\phib_j^{(l)} = \phib_i^{(l)}, \quad \rb_{j, i}^{(l)} \leftarrow [\rb_{j, i}^{\prime{(l)}} || 1],\ $ {\bfseries otherwise}
            % \IF{$\rb_{j,i}^{l\prime} \ne [0,\dots0]^\top$}
            %     \STATE $\rb_{j, i}^l \leftarrow [\rb_{j, i}^{l\top} || 0]$
            % \ELSE
            %     \STATE $\rb_{j, i}^l \leftarrow [\rb_{j, i}^{l\top} || 1]$
            % \ENDIF
            \STATE $ \alpha_{j, i, h}^{(l)} \leftarrow \rb_{j, i}^{{(l)}\top} \widetilde{\phib}_h^{(l)} $
            \ENDFOR
            % \STATE $\mathbf{q}_{i,c} \leftarrow \mathbf{Q}_{c}\mathbf{e}_{i,c}/ \lVert \mathbf{Q}_{c}\mathbf{e}_{i,c}\rVert_2$
            % \STATE $\mathbf{k}_{i,c} \leftarrow \mathbf{K}_c \mathbf{e}_{i,c} / \lVert \mathbf{K}_c \mathbf{e}_{i,c}\rVert_2$
            \STATE $\yb_{i}^{(l)} \leftarrow \sum_h\sum_{j \in \Nc^{(l)} {(i)}} \frac{\exp \left( \alpha_{i,j,h}^{(l)}\right) \Wb_{h}^{(l)} \hb_{j}}{z}$
            
        \ENDFOR
        % \FOR{$j \in \Nc_c\left(i \right)$}
        %     \STATE $a_{j,c} \leftarrow \qb_{i,c}^\top \kb_{j,c}$
        %     \STATE $p_{j,c} \leftarrow \frac{\exp \left(a_{j,c} \right)}{\sum_{j^\prime \in \Nc_c\left(i \right)} \exp\left(a_{j^\prime,c} \right)}$
        %     \STATE $\hb_{i,c} \leftarrow \sum_{j \in \Nc_c\left(i\right)} p_{j,c}\Wb_c\hb_{j}$
        % \ENDFOR
    \ENDFOR
    \STATE $\mathbf{\tilde{y}}_{v}^{(l)} \leftarrow \yb_{v}^{(l)} / \lVert \yb_{v}^{(l)}\rVert_2$
    \STATE $s_{v}^{(l)} \leftarrow \frac{\exp \left(\mathbf{z}^\top \mathbf{\tilde{y}}_{v}^{(l)} \right)}{\sum_{l^\prime=0}^{L+1} \exp \left(\mathbf{z}^\top \mathbf{\tilde{y}}_{v}^{(l^\prime)}\right)}$
    \STATE $\widetilde{\hb}_v \leftarrow \sum_{l=0}^{L+1} s_{v}^{(l)}\mathbf{\tilde{y}}_{v}^{(l)}$
\end{algorithmic}
\end{algorithm}
% \begin{algorithm}[t]
%   \caption{Our network (Temp)}
%   \label{alg:pseudocode}
% \begin{algorithmic}[1]
% %   \REQUIRE $G$, $\mathbf{X} \in \mathbf{R}^{n \times d}$\\
% %   \textbf{Network Parameters:} $\mathbf{W}_e \in \mathbf{R}^{d \times d_e}, \mathbf{W}_o \in \mathbf{R}^{d_e \times C}, \alpha^{(k)}, \text{weight of MLP layers}$
% %   \ENSURE $\mathbf{h}_i^{(\text{output})} (i=1, \dots, n)$
% %   \FOR{$v_u \in V$}
%     \STATE $\mathbf{\tilde{z}}_i \leftarrow f\left(v_i \right) \quad \forall i\in V$
%     \STATE $[p_{i,1}\dots p_{i,K}] \leftarrow \text{softmax}\left(\mathbf{W}^\top\mathbf{\tilde{z}}_{i} \right) \quad \forall i \in V$
%     \STATE $\mathbf{\tilde{a}}_k \leftarrow {\sum_{i}p_{i,k}\mathbf{\tilde{z}}_i}/{\sum_{i}p_{i,k}}$
%     \FOR{$l=0$ {\bfseries to} $l=L-1$}
%         \STATE $\mathbf{a}_k^{(l)} \leftarrow {\sum_{i}p_{i,k}\mathbf{h}^{(l)}_i}/{\sum_{i}p_{i,k}}$
%         \STATE $\mathbf{c}_{i,k}^{(l+1)} \leftarrow \sum_{u \in \mathcal{N}(v)} \frac{\exp  \left(\mathbf{z}_u^\top \mathbf{a}_k \right)}{\sum_{k^\prime}\exp\left(\mathbf{z}_u^\top \mathbf{a}_{k^\prime} \right)} \mathbf{W}_k \mathbf{h}_u^{(l)}$
%         \STATE $\mathbf{n}_i^{(l+1)} \leftarrow \sum_k \mathbf{c}_{i,k}^{(l+1)}$
%         \STATE $\mathbf{e}_i^{(l+1)} \leftarrow \sum_k \frac{\exp  \left(\mathbf{z}_i^\top \mathbf{a}_k \right)}{\sum_{k^\prime}\exp\left(\mathbf{z}_i^\top \mathbf{a}_{k^\prime} \right)}\mathbf{W}^\prime \mathbf{a}_k^{(l)}$
%         \STATE $\mathbf{h_i}^{(l+1)} \leftarrow \mathbf{n}_i^{(l+1)} + \mathbf{e}_i^{(l+1)}$
%   \ENDFOR
% \end{algorithmic}
% \end{algorithm}

==> Algorithms/pseudocode4.tex <==
% 나중 수정
\begin{algorithm}[t]
  \caption{Deformable Graph Convolutional Networks}
  \label{alg_sup:pseudocode}
\begin{flushleft}
    \textbf{Input: } Graph: $G=\left(V, E \right)\ $; Latent Neighborhood Graph: $\Gc^{(l)}$; Node features $\mathbf{x}_v\in \Rbb^{d_x}$; Smoothed input features: $\eb_v^{(l)}\in \Rbb^{d_x}$   \\
    \textbf{Output: } $\widetilde{\hb}_v \in \Rbb^{d_y}$\\
    \textbf{Parameters:} $\Wb \in \Rbb^{d_h \times d_x}$; $\mathbf{W}_\phi^{(l)}\in \Rbb^{d_\phi \times d_x}$; $\Wb_k^{(l)} \in \Rbb^{d_y \times d_h}; \widetilde{\phib}^{(l)}_k \in \Rbb^{d_{\phi+1}}$\\
    % \textbf{Network PArameters:}  params of $\psi_{\text{LN}}(\cdot)$ \\
\end{flushleft}
\begin{algorithmic}[1]
%   \REQUIRE $G$, $\mathbf{X} \in \mathbf{R}^{n \times d}$\\
%   {\bfseries Network Parameters:} $\mathbf{W}_e \in \mathbf{R}^{d \times d_e}, \mathbf{W}_o \in \mathbf{R}^{d_e \times C}, \alpha^{(k)}, \text{weight of MLP layers}$
%   \ENSURE $\mathbf{h}_i^{(\text{output})} (i=1, \dots, n)$

%   \FOR{$v_u \in V$}
    \STATE $\hb_v \leftarrow \sigma \left(\Wb \xb_v\right), \forall v \in V$
    \FOR{$l=0$ {\bfseries to} $l=L+1$}
        \STATE $\phib_{v}^{(l)} \leftarrow \Wb_\phi^{(l)} \mathbf{e}_{v}^{(l)}$
        %\FOR{$i \in \left\{v\right\} \cup \left\{u : \left(u,v\right) \in \Ec^{(l)}\right\}$}
        \FOR{$u \in \widetilde{\Nc}^{\left (l \right)}\left(v \right)$}
            \STATE $\rb^{\prime (l)}_{u, v} \leftarrow \left({\phib_{u}^{(l)} - \phib_{v}^{(l)}}\right)/{\lVert \phib_{u}^{(l)} - \phib_{v}^{(l)} \rVert_2}$
            \STATE $\rb_{u, v}^{(l)} \leftarrow [\rb_{u, v}^{\prime(l)} || 0],\ $ {\bfseries  if} $\phib_u^{(l)} = \phib_v^{(l)}, \quad \rb_{u, v}^{(l)} \leftarrow [\rb_{u, v}^{\prime{(l)}} || 1],\ $ {\bfseries otherwise}
            % \IF{$\rb_{j,i}^{l\prime} \ne [0,\dots0]^\top$}
            %     \STATE $\rb_{j, i}^l \leftarrow [\rb_{j, i}^{l\top} || 0]$
            % \ELSE
            %     \STATE $\rb_{j, i}^l \leftarrow [\rb_{j, i}^{l\top} || 1]$
            % \ENDIF
            \ENDFOR
            % \STATE $\mathbf{q}_{i,c} \leftarrow \mathbf{Q}_{c}\mathbf{e}_{i,c}/ \lVert \mathbf{Q}_{c}\mathbf{e}_{i,c}\rVert_2$
            % \STATE $\mathbf{k}_{i,c} \leftarrow \mathbf{K}_c \mathbf{e}_{i,c} / \lVert \mathbf{K}_c \mathbf{e}_{i,c}\rVert_2$
            \STATE $\yb_{v}^{(l)} \leftarrow \sum_{u \in \widetilde {\Nc}^{(l)} {(v)}} \sum_k\frac{\exp \left( \rb_{u, v}^{{(l)}\top} \widetilde{\phib}_k^{(l)}\right) \Wb_{k}^{(l)} \hb_{u}}{\sum_{u^\prime}\exp \left( \rb_{u^\prime, v}^{{(l)}\top} \widetilde{\phib}_k^{(l)}\right)}$
            
        
        % \FOR{$j \in \Nc_c\left(i \right)$}
        %     \STATE $a_{j,c} \leftarrow \qb_{i,c}^\top \kb_{j,c}$
        %     \STATE $p_{j,c} \leftarrow \frac{\exp \left(a_{j,c} \right)}{\sum_{j^\prime \in \Nc_c\left(i \right)} \exp\left(a_{j^\prime,c} \right)}$
        %     \STATE $\hb_{i,c} \leftarrow \sum_{j \in \Nc_c\left(i\right)} p_{j,c}\Wb_c\hb_{j}$
        % \ENDFOR
    \ENDFOR
    \STATE $\mathbf{\tilde{y}}_{v}^{(l)} \leftarrow \yb_{v}^{(l)} / \lVert \yb_{v}^{(l)}\rVert_2$
    \STATE $s_{v}^{(l)} \leftarrow \frac{\exp \left(\mathbf{z}^\top \mathbf{\tilde{y}}_{v}^{(l)} \right)}{\sum_{l^\prime=0}^{L+1} \exp \left(\mathbf{z}^\top \mathbf{\tilde{y}}_{v}^{(l^\prime)}\right)}$
    \STATE $\widetilde{\hb}_v \leftarrow \sum_{l=0}^{L+1} s_{v}^{(l)}\mathbf{\tilde{y}}_{v}^{(l)}$
\end{algorithmic}
\end{algorithm}
% \begin{algorithm}[t]
%   \caption{Our network (Temp)}
%   \label{alg:pseudocode}
% \begin{algorithmic}[1]
% %   \REQUIRE $G$, $\mathbf{X} \in \mathbf{R}^{n \times d}$\\
% %   \textbf{Network Parameters:} $\mathbf{W}_e \in \mathbf{R}^{d \times d_e}, \mathbf{W}_o \in \mathbf{R}^{d_e \times C}, \alpha^{(k)}, \text{weight of MLP layers}$
% %   \ENSURE $\mathbf{h}_i^{(\text{output})} (i=1, \dots, n)$
% %   \FOR{$v_u \in V$}
%     \STATE $\mathbf{\tilde{z}}_i \leftarrow f\left(v_i \right) \quad \forall i\in V$
%     \STATE $[p_{i,1}\dots p_{i,K}] \leftarrow \text{softmax}\left(\mathbf{W}^\top\mathbf{\tilde{z}}_{i} \right) \quad \forall i \in V$
%     \STATE $\mathbf{\tilde{a}}_k \leftarrow {\sum_{i}p_{i,k}\mathbf{\tilde{z}}_i}/{\sum_{i}p_{i,k}}$
%     \FOR{$l=0$ {\bfseries to} $l=L-1$}
%         \STATE $\mathbf{a}_k^{(l)} \leftarrow {\sum_{i}p_{i,k}\mathbf{h}^{(l)}_i}/{\sum_{i}p_{i,k}}$
%         \STATE $\mathbf{c}_{i,k}^{(l+1)} \leftarrow \sum_{u \in \mathcal{N}(v)} \frac{\exp  \left(\mathbf{z}_u^\top \mathbf{a}_k \right)}{\sum_{k^\prime}\exp\left(\mathbf{z}_u^\top \mathbf{a}_{k^\prime} \right)} \mathbf{W}_k \mathbf{h}_u^{(l)}$
%         \STATE $\mathbf{n}_i^{(l+1)} \leftarrow \sum_k \mathbf{c}_{i,k}^{(l+1)}$
%         \STATE $\mathbf{e}_i^{(l+1)} \leftarrow \sum_k \frac{\exp  \left(\mathbf{z}_i^\top \mathbf{a}_k \right)}{\sum_{k^\prime}\exp\left(\mathbf{z}_i^\top \mathbf{a}_{k^\prime} \right)}\mathbf{W}^\prime \mathbf{a}_k^{(l)}$
%         \STATE $\mathbf{h_i}^{(l+1)} \leftarrow \mathbf{n}_i^{(l+1)} + \mathbf{e}_i^{(l+1)}$
%   \ENDFOR
% \end{algorithmic}
% \end{algorithm}

==> Figure_tex/analysis.tex <==
\begin{figure}[t]
\centering
% \includesvg[width=0.5\textwidth]{Figures/score_deform27.svg}
\includegraphics[width=0.5\textwidth]{Figures/analysis_temp_b.png}
\caption{
The \textcolor{red}{attention score $s^{(l)}$ for \textit{latent neighborhood graph}} $\Gc^{(l)}$. 
Datasets above the dash line are heterophilic graphs and the others homophilic graph datasets.
}
\label{fig:temp_hop-analysis}
\end{figure}

==> Figure_tex/analysis2.tex <==
\begin{figure}[t]
\centering
% \includesvg[width=0.5\textwidth]{Figures/score_deform27.svg}
\includegraphics[width=0.7\textwidth]{Figures/analysis2.png}
% \includesvg[width=0.5\textwidth]{Figures/analysis2.svg
\caption{Receptive field for each target nodes on Cora dataset.
}
\label{fig:recep}
\end{figure}

==> Figure_tex/analysis3.tex <==
\begin{wrapfigure}{tr}{0.35\textwidth}
% \centering
% \includesvg[width=0.5\textwidth]{Figures/score_deform27.svg}
\includegraphics[width=0.35\textwidth]{Figures/analysis_temp_b.png}
\caption{
The \textcolor{red}{attention score $s^{(l)}$ for \textit{latent neighborhood graph}} $\Gc^{(l)}$. 
Datasets above the dash line are heterophilic graphs and the others homophilic graph datasets.
\textcolor{red}{Draw the Dashline between text `Cornell' and  `Citeseer'.}}
\label{fig:temp_hop-analysis}
\end{wrapfigure}

==> Figure_tex/deform.tex <==
% \begin{figure}[t]
% \centering
% \subfigure[Graph Convolution]{
% \label{fig:graphconv}
% \includegraphics[width=0.45\textwidth]{Figures/gc6.png}
% }
% \subfigure[Deformable Graph Convolution]{
% \label{fig:deformablegraphconv}
% \includegraphics[width=0.45\textwidth]{Figures/deform_gc6.png}
% }
% \caption{Comparison between original graph convolution~(a) and Deformable Graph Convolution~(b).
% In the original graph convolution, each node gets messages from neighborhoods in proportion to node degree with a single linear projection, whereas Deformable GConv uses node-wise deformed filters (center hole blank circles) to get messages from neighborhoods in an attention manner. Here, the number of filters can vary.}
% \caption{Comparison between original GCN and Deformable GCN. 
% In the original GCN, node $v$ get messages from neighborhoods $N\left(v\right)$ in proportion to node degree with single linear projection, whereas Deformable GCN uses node-wise deformed filters to get messages from neighborhoods $\widetilde{\Nc}^{(l)}(v)$ on a latent graph.}
% selecively influenced 라고 써도 될까?
% Edge 굵기나 feature 색깔도 언급을 해줘야 할까?
% \label{fig:figure4}
% \end{figure}
\begin{figure*}[t]
\centering
\includegraphics[width=1\textwidth]{Figures/fig2.png}
\caption{
\jhp{Comparison between original graph convolution~(left) and Deformable Graph Convolution~(right).
In the original graph convolution, the same linear transformation is applied for all the relations in the neighborhood for aggregating, whereas Deformable GConv adaptively transforms messages from neighborhoods depending on the relation in the position space.}
% \jyp{Before the beginning of training, latent neighborhood graphs, $\{\Gc^{(l)}\}_{l=1}^{L+1},$ are constructed for generating neighborhood $\{\widetilde{\Nc}^{(l)}\left(v \right)\}_{l=1}^{L+1}$ of a node $v$.}
% Then, Deformable Graph Convolution~(DGConv) is applied to aggregate messages within $\widetilde{\Nc}^{(l)}\left(v \right)$. 
% Then, each output of DGconv is adaptiely aggregated using a simple attention mechanism to learn node representation. }
% Latent neighborhood graphs are constructed in a way that updates features from c-hop aggregation and chooses neighbors of each node in a top-k manner ($0th \sim Lth$ latent graph).
% Here we also use additional latent graph as original graph ($L+1th$ latent graph).
% For within each latent graph, nodes softly aggregates messages from neighbors by using deformable graph convolution (green box) and internally aggregated nodes adaptively aggregate their own messages from every hop (yellow box).}
% \caption{\textbf{Overall structure of our framework.} Our framework leverages the latent graphs for multiple hops to determine which messages of them would be effective to update the node embeddings. Latent graphs are constructed in a way that updates features from c-hop aggregation and chooses neighbors of each node in a top-k manner. For within each latent graph, nodes adaptively aggregates messages by using their own relationship between neighbors and intra-aggregated nodes go through one more adaptive aggregation between graphs. }
%\caption{\textbf{Overall structure of our framework.} Our framework leverages the latent graphs for multiple hops to determine which messages of them would be effective to update the node embeddings. Latent neighborhood graphs are constructed in a way that updates features from c-hop aggregation and chooses neighbors of each node in a top-k manner. For within each latent graph, nodes softly  aggregates messages from neighbors by using deformable convolution and internally aggregated nodes at every hop go through one more adaptive aggregation between graphs.}
}
\label{fig:deform}
\end{figure*}

==> Figure_tex/mixed.tex <==
\begin{figure}[t]
\centering
\subfigure[Attention score.]{
\label{fig:temp_hop-analysis}
\includegraphics[width=0.45\textwidth]{Figures/analysis_temp_b.png}
}
\hspace{0.7cm}
\subfigure[Receptive field for each target nodes.]{
\label{recep}
\includegraphics[width=0.45\textwidth]{Figures/analysis2.png}
}
% \subfigure[Pubmed]{
% \includegraphics[width=0.30\textwidth]{Figures/abblation_temp2.png}
% }
\caption{Analysis on Deformable GCNs. The left figure is the \textcolor{black}{attention score $s^{(l)}$ for \textit{latent neighborhood graph}} $\Gc^{(l)}$. 
Datasets above the dash line are heterophilic graphs and the others homophilic graph datasets.
The right figure is the visualization of the receptive field of each target node on Cora dataset.
}
\label{fig:mixed}
% selecively influenced 라고 써도 될까?
% Edge 굵기나 feature 색깔도 언급을 해줘야 할까?
\end{figure}

==> Figure_tex/sup_homophily_heterophily.tex <==
\begin{figure*}[ht!]
\centering
\subfigure[Texas : $\mathbb{E}(h_{\text{nbh}})=0.06$]{
\includegraphics[width=0.3\textwidth]{Figure_sup/texas.png}
}
\subfigure[Wisconsin : $\mathbb{E}(h_{\text{nbh}})=0.16$]{
\includegraphics[width=0.3\textwidth]{Figure_sup/wisconsin.png}
}
\subfigure[Actor : $\mathbb{E}(h_{\text{nbh}})=0.22$]{
\includegraphics[width=0.3\textwidth]{Figure_sup/film.png}
}
\subfigure[Chameleon : $\mathbb{E}(h_{\text{nbh}})=0.25$]{
\includegraphics[width=0.3\textwidth]{Figure_sup/chameleon.png}
}
\subfigure[Squirrel : $\mathbb{E}(h_{\text{nbh}})=0.22$]{
\includegraphics[width=0.3\textwidth]{Figure_sup/squirrel.png}
}
\subfigure[Cornell : $\mathbb{E}(h_{\text{nbh}})=0.30$]{
\includegraphics[width=0.3\textwidth]{Figure_sup/cornell.png}
}
\subfigure[Citeseer : $\mathbb{E}(h_{\text{nbh}})=0.72$]{
\includegraphics[width=0.3\textwidth]{Figure_sup/citeseer.png}
}
\subfigure[Pubmed : $\mathbb{E}(h_{\text{nbh}})=0.79$]{
\includegraphics[width=0.3\textwidth]{Figure_sup/pubmed.png}
}
\subfigure[Cora : $\mathbb{E}(h_{\text{nbh}})=0.83$]{
\includegraphics[width=0.3\textwidth]{Figure_sup/cora.png}
}
% \vsapce{10cm}
\caption{Neighborhood-based homophily ratio $h_{\text{nbh}}$ on each dataset.
}

% selecively influenced 라고 써도 될까?
% Edge 굵기나 feature 색깔도 언급을 해줘야 할까?
\label{fig_sup:dataset}
\end{figure*}

==> Figure_tex/sup_noreg.tex <==
\begin{figure}[t]
\centering

\includegraphics[width=0.99\linewidth]{Figure_sup/no_reg.png}

% \subfigure[Pubmed]{
% \includegraphics[width=0.30\textwidth]{Figures/abblation_temp2.png}
% }
\caption{The visualization of kernel vectors $\widetilde{\phib}_k$ and deformed kernel vectors $\widetilde{\phib}_k + \Delta_k\left(\eb_v\right)$ on position space when training without regularizations. 
% The intensity of the color of each node is associated with the intensity of each node. 
}
\label{fig_sup:noreg}
% selecively influenced 라고 써도 될까?
% Edge 굵기나 feature 색깔도 언급을 해줘야 할까?
\end{figure}

==> Tables/Main_table_old.tex <==
\begin{table*}[t]
    \centering
    \setlength{\tabcolsep}{2.5pt}    
    % \begin{adjustbox}{width=1.0\textwidth}    
    \begin{tabular}{l|cccccc|ccc}
    % \begin{tabular}{l|cccccc|ccc}
    \toprule
    % \textbf{Dataset}   & \textbf{Texas} & \textbf{Wisconsin} & \textbf{Actor} & \textbf{Squirrel} & \textbf{Chameleon} & \textbf{Cornell} & \textbf{Citeseer} & \textbf{Pubmed} & \textbf{Cora} \\
    \textbf{Dataset}   & \textbf{Texas} & \textbf{Wisconsin} & \textbf{Actor} & \textbf{Squirrel} & \textbf{Chameleon} & \textbf{Cornell} & \textbf{Citeseer} & \textbf{Pubmed} & \textbf{Cora} \\
    \textbf{Hom. ratio} $h$       &  \textbf{0.11} &      \textbf{0.21} &  \textbf{0.22} &     \textbf{0.22} &    \textbf{0.23} &    \textbf{0.30} & \textbf{0.74} &  \textbf{0.80} & \textbf{0.81} \\
    \midrule
    \midrule
    MLP       & 82.16{\scriptsize$\pm$4.26} &    84.90{\scriptsize$\pm$2.93} &  36.78{\scriptsize$\pm$0.91} &     30.77{\scriptsize$\pm$2.71} &  47.87{\scriptsize$\pm$2.11} &   81.08{\scriptsize$\pm$5.84} & 72.86{\scriptsize$\pm$2.29} &87.62{\scriptsize$\pm$0.31} & 75.09{\scriptsize$\pm$2.34}\\
    GCN       & 64.32{\scriptsize$\pm$4.19} &    62.94{\scriptsize$\pm$6.76} &  30.47{\scriptsize$\pm$1.04} &     46.65{\scriptsize$\pm$1.60} &  64.98{\scriptsize$\pm$1.12} &   60.27{\scriptsize$\pm$3.83} & 76.66{\scriptsize$\pm$1.80} &87.59{\scriptsize$\pm$0.58} & 87.44{\scriptsize$\pm$1.34}\\
    GAT       & 60.81{\scriptsize$\pm$7.46} &    64.31{\scriptsize$\pm$5.61} &  29.92{\scriptsize$\pm$0.69} &     45.47{\scriptsize$\pm$2.23} &  66.56{\scriptsize$\pm$1.60} &   59.46{\scriptsize$\pm$2.55} & 76.54{\scriptsize$\pm$1.62} &86.55{\scriptsize$\pm$0.55} & 87.46{\scriptsize$\pm$1.24}\\
    ChebyNet & 76.49{\scriptsize$\pm$5.56} &    77.84{\scriptsize$\pm$5.31} &  35.03{\scriptsize$\pm$1.18} &     45.42{\scriptsize$\pm$0.10} &  61.80{\scriptsize$\pm$1.92} &   72.97{\scriptsize$\pm$7.43} & 76.20{\scriptsize$\pm$1.81} &89.16{\scriptsize$\pm$0.49} & 83.44{\scriptsize$\pm$3.29}\\    
    JKNet     & 62.97{\scriptsize$\pm$8.36} &    60.78{\scriptsize$\pm$5.31} &  30.78{\scriptsize$\pm$0.97} &     53.78{\scriptsize$\pm$2.01} &  68.53{\scriptsize$\pm$2.57} &   59.19{\scriptsize$\pm$3.48} & 76.05{\scriptsize$\pm$1.61} &88.64{\scriptsize$\pm$0.55} & 87.12{\scriptsize$\pm$1.30}\\
    MixHop     & 83.78{\scriptsize$\pm$5.41} &    85.10{\scriptsize$\pm$4.15} &  33.80{\scriptsize$\pm$1.43} &     39.32{\scriptsize$\pm$3.49} &  63.09{\scriptsize$\pm$1.73} &  81.08{\scriptsize$\pm$7.43}  & 75.86{\scriptsize$\pm$1.93} &89.02{\scriptsize$\pm$0.42} & 87.20{\scriptsize$\pm$1.37}\\
    Geom-GCN  & 68.11{\scriptsize$\pm$4.90} &    64.51{\scriptsize$\pm$4.08} &  31.48{\scriptsize$\pm$1.03} &     38.00{\scriptsize$\pm$0.97} &  60.99{\scriptsize$\pm$2.80} &   60.54{\scriptsize$\pm$5.73} & \textbf{77.48{\scriptsize$\pm$1.40}} &\textbf{89.51{\scriptsize$\pm$0.54}} & 85.51{\scriptsize$\pm$1.49}\\    
    $\text{H}_2$GCN     & 82.16{\scriptsize$\pm$6.65} &    86.67{\scriptsize$\pm$3.51} &  36.96{\scriptsize$\pm$0.88} &     54.51{\scriptsize$\pm$1.52} &  65.42{\scriptsize$\pm$2.55} &   80.54{\scriptsize$\pm$6.08} & 77.05{\scriptsize$\pm$1.45} &89.38{\scriptsize$\pm$0.42} & \textbf{87.48{\scriptsize$\pm$1.50}}\\
    \midrule
    Deformable GCN & \textbf{84.32{\scriptsize$\pm$5.52}} &  \textbf{87.06{\scriptsize$\pm$3.48}} &  \textbf{37.07{\scriptsize$\pm$1.28}} &  \textbf{62.56{\scriptsize$\pm$2.12}} &  \textbf{70.90{\scriptsize$\pm$1.80}}  &  \textbf{85.95{\scriptsize$\pm$4.38}} &76.83{\scriptsize$\pm$1.85} & 89.49{\scriptsize$\pm$0.47} & \textbf{87.48{\scriptsize$\pm$1.33}}\\
    \bottomrule
  \end{tabular}
  \caption{Evaluation results on node classification task~(Accuracy)}
  \label{tab:main table}
%   \end{adjustbox}
\end{table*}
    % Ours      & 80.54 &    86.67 &  36.93 &     \textbf{60.03} &  70.66  & 81.89 & 76.75 & 89.13 & 87.51\\

==> Tables/ablation.tex <==
% \begin{table}[t]
%     \centering
%     % \setlength{\tabcolsep}{3.5pt}  
%     % \begin{adjustbox}{width=0.45\textwidth}
%     \begin{tabular}{l|cc}
%     % \begin{tabular}{l|cccccc|ccc}
%     \toprule
%     % \textbf{Dataset}   & \textbf{Texas} & \textbf{Wisconsin} & \textbf{Actor} & \textbf{Squirrel} & \textbf{Chameleon} & \textbf{Cornell} & \textbf{Citeseer} & \textbf{Pubmed} & \textbf{Cora} \\
%     \textbf{Dataset}   & w/o Reg. & w/ Reg.  \\
%     \midrule
%     \midrule
%     Wisconsin      & 84.12 &    \textbf{87.06}  \\
%     Actor     &  36.67   &  \textbf{37.07}        \\
%     Squirrel & 60.31 &    \textbf{62.56}  \\
%     Pubmed   & 89.02 &    \textbf{89.49} \\
%     \bottomrule
%   \end{tabular}
%   \caption{Ablation.}
%   \label{tab:abl}
% %   \end{adjustbox}
% \end{table}

\begin{table}[t]
    \centering
    % \setlength{\tabcolsep}{3.5pt}  
    % \begin{adjustbox}{width=0.45\textwidth}
    \begin{tabular}{l|cccc}
    % \begin{tabular}{l|cccccc|ccc}
    \toprule
    % \textbf{Dataset}   & \textbf{Texas} & \textbf{Wisconsin} & \textbf{Actor} & \textbf{Squirrel} & \textbf{Chameleon} & \textbf{Cornell} & \textbf{Citeseer} & \textbf{Pubmed} & \textbf{Cora} \\
    \textbf{Dataset}   & Wisconsin & Actor & Squirrel & Pubmed  \\
    \midrule
    w/o Reg.      & 84.12        & 36.67 & 60.31 & 89.02    \\
    w/ Reg.       &\textbf{87.06} & \textbf{37.07}  &    \textbf{62.56} & \textbf{89.49}  \\
    \bottomrule
  \end{tabular}
  \caption{Ablation.}
  \label{tab:abl}
%   \end{adjustbox}
\end{table}
    % Ours      & 80.54 &    86.67 &  36.93 &     \textbf{60.03} &  70.66  & 81.89 & 76.75 & 89.13 & 87.51\\
    
% \begin{figure}
% \begin{float}
% \ffigbox{
% \centering
% \subfigure[Wisconsin ]{
% \includegraphics[width=0.36\textwidth]{Figures/abblation_temp1.png}
% }
% \hspace{0.7cm}
% \subfigure[Pubmed]{
% \includegraphics[width=0.36\textwidth]{Figures/abblation_temp2.png}
% }
% \subfigure[Pubmed]{
% \includegraphics[width=0.30\textwidth]{Figures/abblation_temp2.png}
% }
% selecively influenced 라고 써도 될까?
% Edge 굵기나 feature 색깔도 언급을 해줘야 할까?
% \label{fig:abl}
% }
% {\caption{Ablation study on deformable graph convolution.
% We compare \textbf{Defomrable GCN} and the model without deformation~(\textbf{w/o Deformation}), which uses only kernel vectors on Wisconsin and Pubmed datasets according to number of the kernel vectors.}
% }
% \capbtabbox{
%     \begin{tabular}{l|ccc}
%     % \begin{tabular}{l|cccccc|ccc}
%     \toprule
%     % \textbf{Dataset}   & \textbf{Texas} & \textbf{Wisconsin} & \textbf{Actor} & \textbf{Squirrel} & \textbf{Chameleon} & \textbf{Cornell} & \textbf{Citeseer} & \textbf{Pubmed} & \textbf{Cora} \\
%     \textbf{Dataset}   & \textbf{Texas} & \textbf{Wisconsin} & \textbf{Actor}  \\
%     \textbf{Hom. ratio} $h$       &  \textbf{0.11} &      \textbf{0.21} &  \textbf{0.22}  \\
%     \midrule
%     \midrule
%     Wisconsin      & 82.16 &    84.90 &  36.78     \\
%     Chameleon & 76.49 &    77.84 &  35.03  \\
%     Pubmed   & 62.70 &    61.57 &  30.47 \\
%     \bottomrule
%   \end{tabular}
% }
% {\caption{possible}
% }
% \end{float}
% \end{figure}    


==> Tables/rebuttal_emb.tex <==
\begin{table}[h]
    \centering
    \caption{Ablation study.}
    \label{tab_sup:ablation}
    \setlength{\tabcolsep}{2.5pt}    
    \begin{adjustbox}{width=1.0\textwidth}    
    \begin{tabular}{l|cccccc|ccc}
    % \begin{tabular}{l|cccccc|ccc}
    \toprule
    % \textbf{Dataset}   & \textbf{Texas} & \textbf{Wisconsin} & \textbf{Actor} & \textbf{Squirrel} & \textbf{Chameleon} & \textbf{Cornell} & \textbf{Citeseer} & \textbf{Pubmed} & \textbf{Cora} \\
    \textbf{Dataset}   & \textbf{Texas} & \textbf{Wisconsin} & \textbf{Actor} & \textbf{Squirrel} & \textbf{Chameleon} & \textbf{Cornell} & \textbf{Citeseer} & \textbf{Pubmed} & \textbf{Cora} \\
    \midrule
    \midrule
    w/o deformation & 77.057 &    84.90 &  36.72 &     62.32 &  70.46 &   78.38 & 76.75 &88.67 & 86.80\\

    Deformable GCN  & \textbf{84.32} &  \textbf{87.06} &  \textbf{37.07} &  \textbf{62.56} &  \textbf{70.90}  &  \textbf{85.95} &\textbf{76.83} & \textbf{89.49} & \textbf{87.48}\\
    \bottomrule
  \end{tabular}
  \end{adjustbox}
\end{table}

==> Tables/rebuttal_latentgraphs.tex <==
\vspace{-10pt}
\begin{table}[h!]
    \centering
    % \setlength{\tabcolsep}{3.5pt}  
    % \begin{adjustbox}{width=0.45\textwidth}
    % \setlength{\tabcolsep}{4pt}
    \small{
    \begin{tabular}{c|cccc}
    % \begin{tabular}{l|cccccc|ccc}
    \toprule
    % \textbf{Dataset}   & \textbf{Texas} & \textbf{Wisconsin} & \textbf{Actor} & \textbf{Squirrel} & \textbf{Chameleon} & \textbf{Cornell} & \textbf{Citeseer} & \textbf{Pubmed} & \textbf{Cora} \\
    & \multicolumn{4}{c}{$L$}\\
    % \cmidrule{2-5}
    Dataset              & 1 &  2 & 3 & 4   \\
    \midrule
    Pubmed       & 89.02 &   89.37& 89.45 &\textbf{89.49} \\
    Wisconsin     &  85.99    &   86.47   & 86.47 &\textbf{87.06}   \\
    \bottomrule
  \end{tabular}
  }
  \vspace{-7pt}
  \caption{\small Ablation study for the number of latent graphs $L$.}
%   such as node2vec~\cite{grover2016node2vec} and Poincare embedding~\cite{nickel2018learning} }
  \label{tab_reb:numlayer_abl}
%   \end{adjustbox}
\vspace{-10pt}
\end{table}

==> Tables/sup_ablation.tex <==
\begin{table}[h]
    \centering
    \caption{Ablation study.}
    \label{tab_sup:ablation}
    \setlength{\tabcolsep}{2.5pt}    
    \begin{adjustbox}{width=1.0\textwidth}    
    \begin{tabular}{l|cccccc|ccc}
    % \begin{tabular}{l|cccccc|ccc}
    \toprule
    % \textbf{Dataset}   & \textbf{Texas} & \textbf{Wisconsin} & \textbf{Actor} & \textbf{Squirrel} & \textbf{Chameleon} & \textbf{Cornell} & \textbf{Citeseer} & \textbf{Pubmed} & \textbf{Cora} \\
    \textbf{Dataset}   & \textbf{Texas} & \textbf{Wisconsin} & \textbf{Actor} & \textbf{Squirrel} & \textbf{Chameleon} & \textbf{Cornell} & \textbf{Citeseer} & \textbf{Pubmed} & \textbf{Cora} \\
    \midrule
    \midrule
    w/o deformation & 77.03 &    84.90 &  36.72 &     62.32 &  70.46 &   78.38 & 76.75 &88.67 & 86.80\\

    Deformable GCN  & \textbf{84.32} &  \textbf{87.06} &  \textbf{37.07} &  \textbf{62.56} &  \textbf{70.90}  &  \textbf{85.95} &\textbf{76.83} & \textbf{89.49} & \textbf{87.48}\\
    \bottomrule
  \end{tabular}
  \end{adjustbox}
\end{table}

==> Tables/sup_aggr_table.tex <==
\begin{table}[t]
    \centering
    \scriptsize
    % \setlength{\tabcolsep}{3.5pt}  
    % \begin{adjustbox}{width=0.45\textwidth}
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{c|cccccc}
    % \begin{tabular}{l|cccccc|ccc}
    \toprule
    % \textbf{Dataset}   & \textbf{Texas} & \textbf{Wisconsin} & \textbf{Actor} & \textbf{Squirrel} & \textbf{Chameleon} & \textbf{Cornell} & \textbf{Citeseer} & \textbf{Pubmed} & \textbf{Cora} \\
    &\multicolumn{6}{c}{Dataset}\\
    Aggr. in (7)& Wisconsin & Actor & Squirrel & Cornell & Pubmed & Cora  \\
    \midrule
    Sum        & 84.51 & 36.27  &   57.39 & 82.7 & 87.95 & 87.16\\
    Attention        & \textbf{87.06} & \textbf{37.07} & \textbf{62.56} & \textbf{85.95} & \textbf{89.49} & \textbf{87.48}    \\
    \bottomrule
  \end{tabular}
  \caption{\label{tab_sup:layer_abl} Comparison of our attention mechanism scheme in Equation (7) of the main paper $\left(\sum_l s_v^{(l)}\widetilde{\yb}_v^{(l)} \right)$ with a simple summation $\left(\sum_l \widetilde{\yb}_v^{(l)} \right)$ on six datasets.}
%   such as node2vec~\cite{grover2016node2vec} and Poincare embedding~\cite{nickel2018learning} }
  \label{tab_sup:aggr_abl}
%   \end{adjustbox}
\end{table}

% \begin{table}[t]
%     \centering
%     % \setlength{\tabcolsep}{3.5pt}  
%     % \begin{adjustbox}{width=0.45\textwidth}
%     \setlength{\tabcolsep}{4pt}
%     \begin{tabular}{c|cccccc}
%     % \begin{tabular}{l|cccccc|ccc}
%     \toprule
%     % \textbf{Dataset}   & \textbf{Texas} & \textbf{Wisconsin} & \textbf{Actor} & \textbf{Squirrel} & \textbf{Chameleon} & \textbf{Cornell} & \textbf{Citeseer} & \textbf{Pubmed} & \textbf{Cora} \\
%     Positional&\multicolumn{3}{c}{Dataset}\\
%     embedding& Wisconsin & Actor & Squirrel   \\
%     \midrule
%     Sum        & 84.51 & 36.27  &   57.39 \\
%     Mean        & 87.06 & 37.07 & 62.56     \\
%     \midrule
%     \midrule
%     Positional&\multicolumn{3}{c}{Dataset}\\
%      & Cornell & Pubmed & Cora \\
%     \midrule
%      Sum& 82.7 & 87.95 & 87.16 \\
%      Mean& 85.95 & 89.49 & 87.48 \\
%     \bottomrule
%   \end{tabular}
%   \caption{Comparison of our node positional embeddings with other node embedding methods on four datasets.}
% %   such as node2vec~\cite{grover2016node2vec} and Poincare embedding~\cite{nickel2018learning} }
%   \label{tab:norm_abl}
% %   \end{adjustbox}
% \end{table}

==> Tables/sup_bigdata.tex <==
\begin{table}[h]
    \centering
    \caption{Evaluation results on large graph dataset.}
    \label{tab_sup:large}
    % \setlength{\tabcolsep}{3.5pt}  
    % \begin{adjustbox}{width=0.5\textwidth}
    \begin{tabular}{l|cc}
    % \begin{tabular}{l|cccccc|ccc}
    \toprule
    % \textbf{Dataset}   & \textbf{Texas} & \textbf{Wisconsin} & \textbf{Actor} & \textbf{Squirrel} & \textbf{Chameleon} & \textbf{Cornell} & \textbf{Citeseer} & \textbf{Pubmed} & \textbf{Cora} \\
    \textbf{Dataset}   & YelpChi & arXiv-year  \\
    \midrule
    \midrule
    MLP             &  82.61   &  36.51       \\
    GCN              & 60.41   &  42.94  \\
    GAT              & 58.45   &  39.17        \\
    DeformableGCN   &  \textbf{77.04} &  \textbf{44.72} \\
    \bottomrule
  \end{tabular}
%   \end{adjustbox}
\end{table}

==> Tables/sup_data_stats.tex <==
\begin{table}[h]
  \centering
  \setlength{\tabcolsep}{3.5pt}
  \caption{Large graph dataset statistics.}
  \label{tab_sup:data_statistics}
%   \begin{adjustbox}{width=1.0\textwidth}
  \begin{tabular}{c|cccccc}
  \toprule
    \textbf{Dataset}    & \textbf{\# Classes}  &  \textbf{\# Nodes}  & \textbf{\# Edges} & \textbf{\# Features} & \textbf{Avg deg.} & \textbf{Hom. ratio $h$}\\
    \midrule
    \textbf{YelpChi}  & 2 & 45,954 & 3,846,979 &    32 &-- & 0.773 \\
    \textbf{arXiv-year} & 5 & 169,343 & 1,166,243 & 128 & -- & 0.222 \\
    \bottomrule
  \end{tabular}
%   \end{adjustbox}
\end{table}

==> Tables/sup_other.tex <==
\vspace{-15pt}
\begin{table}[h!]
    \centering
    % \setlength{\tabcolsep}{3.5pt}  
    % \begin{adjustbox}{width=0.5\textwidth}
    {\small
    \begin{tabular}{l|cc}
    % \begin{tabular}{l|cccccc|ccc}
    \toprule
    % \textbf{Dataset}   & \textbf{Texas} & \textbf{Wisconsin} & \textbf{Actor} & \textbf{Squirrel} & \textbf{Chameleon} & \textbf{Cornell} & \textbf{Citeseer} & \textbf{Pubmed} & \textbf{Cora} \\
    & \multicolumn{2}{c}{Homophilic Graph Dataset (Hom ratio $h$)}\\
    Models & Computer ($h=0.78$) & Physics ($h=0.93$)  \\
    \midrule
    \midrule
    MLP             &  64.26   &  89.44       \\
    GCN              & 80.04   &  93.27  \\
    GAT              & 81.15   &  93.09        \\
    DeformableGCN   &  \textbf{83.92} &  \textbf{93.32} \\
    \bottomrule
  \end{tabular}
  }
  \vspace{-7pt}
    \caption{\small \label{tab_sup:other}(Same as Table 4 in the supplement)}
%   \end{adjustbox}
  \vspace{-9pt}
\end{table}


% \begin{table}[t]
%     \centering
%     % \setlength{\tabcolsep}{3.5pt}  
%     % \begin{adjustbox}{width=0.5\textwidth}
%     \begin{tabular}{l|cc}
%     % \begin{tabular}{l|cccccc|ccc}
%     \toprule
%     % \textbf{Dataset}   & \textbf{Texas} & \textbf{Wisconsin} & \textbf{Actor} & \textbf{Squirrel} & \textbf{Chameleon} & \textbf{Cornell} & \textbf{Citeseer} & \textbf{Pubmed} & \textbf{Cora} \\
%     Dataset   & Computer & Physics  \\
%     Hom. ratio $h$ &  0.78      & 0.93 \\
%     \midrule
%     \midrule
%     MLP             &  64.26   &  89.44       \\
%     GCN              & 80.04   &  93.27  \\
%     GAT              & 81.15   &  93.09        \\
%     DeformableGCN   &  \textbf{83.92} &  \textbf{93.32} \\
%     \bottomrule
%   \end{tabular}
%     \caption{(Same as Table 4 in the supplement.) Evaluation results on two homophilic graph datasets such as Computer and Physics.}
%     \label{tab_sup:other}
% %   \end{adjustbox}
% \end{table}

==> Tables/sup_time_table.tex <==
\begin{table}[t]
    \centering
    \scriptsize
    % \setlength{\tabcolsep}{3.5pt}  
    % \begin{adjustbox}{width=0.45\textwidth}
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{c|cccccc}
    % \begin{tabular}{l|cccccc|ccc}
    \toprule
    % \textbf{Dataset}   & \textbf{Texas} & \textbf{Wisconsin} & \textbf{Actor} & \textbf{Squirrel} & \textbf{Chameleon} & \textbf{Cornell} & \textbf{Citeseer} & \textbf{Pubmed} & \textbf{Cora} \\
             &\multicolumn{6}{c}{Dataset}\\
    Model    & Wisconsin & Actor & Squirrel & Cornell & Pubmed & Cora  \\
    \midrule
    Geom-GCN        & 92.85 & 908.6  &   3429.0 & 80.4 & 2206.0 & 444.4\\
    Deformable GCN        & \textbf{30.3} & \textbf{57.8} & \textbf{89.8} & \textbf{31.1} & \textbf{69.3} & \textbf{41.7}    \\
    \bottomrule
  \end{tabular}
  \caption{Comparisons of running time~(s) with Geom-GCN and Deformable GCN on six datasets.}
%   such as node2vec~\cite{grover2016node2vec} and Poincare embedding~\cite{nickel2018learning} }
  \label{tab_sup:time_abl}
%   \end{adjustbox}
\end{table}

==> Tables/table_bak.tex <==

\begin{table}[t]
  \centering
  \caption{Mean classification accuracy}
  \label{tab:table_bak}
  \begin{tabular}{l|cccccccc}
    \toprule
    Dataset   & Texas & Wisconsin & Actor & Squirrel & Chamel. & Cornell & Pubmed & Cora \\
    $h$       &  0.11 &      0.21 &  0.22 &     0.22 &    0.23 &    0.30 &   0.80 & 0.81 \\
    \midrule
    \midrule
    MLP       & 82.16 &    84.90 &  36.78 &     30.77 &  48.07 &   81.08 & 87.62 & 75.33\\
    GCN       & 62.70 &    61.57 &  30.47 &     44.81 &  63.55 &   59.73 & 87.43 & 87.40\\
    GAT       & 60.27 &    60.20 &  30.13 &     45.24 &  66.84 &   59.46 & 86.55 & 87.57\\
    GraphSAGE & 80.81 &    83.14 &  34.91 &     50.77 &  66.16 &   74.32 & 88.54 & 87.83\\
    JKNet     & 61.62 &    60.59 &  30.14 &     53.62 &  67.89 &   59.19 & 88.64 & 87.26\\
    FAGCN     & 84.05 &    83.92 &  35.39 &     41.63 &  62.61 &   ----- & 89.05 & 88.25\\
    H2GCN     & 82.16 &    85.88 &  35.62 &     37.90 &  59.39 &   82.16 & 89.59 & 87.81\\
    Geom-GCN  & 68.11 &    64.51 &  31.63 &     38.14 &  60.99 &   60.54 & 90.05 & 85.51\\
    \midrule
    Ours      & 80.54 &    86.67 &  \textbf{36.93} &     \textbf{60.03} &  70.66  &  81.89 & 89.13 & 87.51\\
    Ours+deform & \textbf{85.14} &  \textbf{87.65} &  36.79 &     59.47 &  \textbf{70.75}  &  \textbf{87.03} & ----- & -----\\
    \bottomrule
  \end{tabular}
\end{table}

==> Tables/twoablation.tex <==
\begin{table}[t]
    \centering
    % \setlength{\tabcolsep}{3.5pt}  
    % \begin{adjustbox}{width=0.45\textwidth}
    \begin{tabular}{cc|cccc}
    % \begin{tabular}{l|cccccc|ccc}
    \toprule
    % \textbf{Dataset}   & \textbf{Texas} & \textbf{Wisconsin} & \textbf{Actor} & \textbf{Squirrel} & \textbf{Chameleon} & \textbf{Cornell} & \textbf{Citeseer} & \textbf{Pubmed} & \textbf{Cora} \\
    Regularizers & Position    & Wisconsin & Actor & Squirrel & Pubmed  \\
    \midrule
       &    & 84.12        & 36.67 & 60.31 & 89.02    \\
    \checkmark  &   & 86.08 & 36.70  &    60.43 & \textbf{89.49}  \\
      &\checkmark   & 86.08        & 36.67 & 61.83 & 89.02    \\
    \checkmark  &\checkmark    &\textbf{87.06} & \textbf{37.07}  &    \textbf{62.56} & \textbf{89.49}  \\
    \bottomrule
  \end{tabular}
  \caption{Ablation study of two regularizer losses ($\Lc_{sep.}, \Lc_{focus}$).}
  \label{tab:reg_abl}
%   \end{adjustbox}
\end{table}


